One Sketch for All: One-Shot Personalized Sketch Segmentation

We present the first one-shot personalized sketch segmentation method. We aim to segment all sketches belonging to the same category provisioned with a single sketch with a given part annotation while (i) preserving the parts semantics embedded in the exemplar, and (ii) being robust to input style and abstraction. We refer to this scenario as personalized. With that, we importantly enable a much-desired personalization capability for downstream fine-grained sketch analysis tasks. To train a robust segmentation module, we deform the exemplar sketch to each of the available sketches of the same category. Our method generalizes to sketches not observed during training. Our central contribution is a sketch-specific hierarchical deformation network. Given a multi-level sketch-strokes encoding obtained via a graph convolutional network, our method estimates rigid-body transformation from the target to the exemplar, on the upper level. Finer deformation from the exemplar to the globally warped target sketch is further obtained through stroke-wise deformations, on the lower level. Both levels of deformation are guided by mean squared distances between the keypoints learned without supervision, ensuring that the stroke semantics are preserved. We evaluate our method against the state-of-the-art segmentation and perceptual grouping baselines re-purposed for the one-shot setting and against two few-shot 3D shape segmentation methods. We show that our method outperforms all the alternatives by more than $10\%$ on average. Ablation studies further demonstrate that our method is robust to personalization: changes in input part semantics and style differences.

==> intro.tex <==
\section{Introduction}
With the appearance of large-scale sketch datasets and recent advances in deep learning, sketch-related research thrives \cite{ Liu_2019_ICCV, 
Ghosh_2019_ICCV, Gao_2020_CVPR,Zheng_2020_CVPR,Lin_2020_CVPR, Liu_2020_ECCV, Liu_F_2020_ECCV}. 
Sketch segmentation in particular is an important capability that underpins the recent focus of fine-grained sketch analysis, such as part-based sketch-based modeling and retrieval \cite{jones2020shapeassembly, li2016fine} \old{or}\anran{and} fine-grained sketch editing \cite{Zou_2018_ECCV, su2020sketchhealer}. 

Existing methods aiming at semantic sketch segmentation rely on the availability of large-scale carefully annotated sketch datasets. 
However, obtaining such annotations for new categories is an extremely labor-intensive task. 
\emph{\old{Moreover, current datasets provide fixed part sketches labeling, disregarding the subjective nature of segmentations}
\new{Moreover, current datasets contain a single set of labels per sketch, disregarding the subjective nature of the segmentation task} \cite{MartinFTM01,perteneder2015cluster} -- 
this impedes downstream applications, not allowing \old{the number of meaningful labels}\new{the labels} to be task-specific.} 
% \anran{not do understand 'and their'???}

In this paper, for the first time, we address the problem of \emph{personalized} sketch segmentation under a one-shot setting, as an attempt to facilitate the fine-grained analysis of sketches. 
Namely, given \old{\emph{one} input sketch that is part annotated}\new{\emph{one} annotated sketch}, we seek to label any number of gallery sketches in a consistent manner \old{by conforming}\new{according} to the same user-defined semantic interpretation, and robustly to differences in drawing style and abstraction between the input and gallery.
We refer to this scenario as \emph{personalized sketch segmentation}.
Fig.~\ref{fig:teaser} offers two working examples where two sketches of different styles and part decomposition were used to segment unseen sketches of the same category consistent with each input semantic segmentation.

\begin{figure}[t]
\vspace{-6pt}
\begin{center}
% \fbox{\rule{0pt}{1.3in} \rule{1.0\linewidth}{0pt}}
   \includegraphics[width=1.0\linewidth]{images/teaser_duck_v2.pdf}
\end{center}
\vspace{-6pt}
   \caption{Given an exemplar annotated sketch, we are able to transfer \old{the}\new{its} labels to any \old{amount}\new{number} of sketches of the same category and achieve task-specific segmentation.
}
\label{fig:teaser}
\vspace{-8pt}
\end{figure}


The problem of one-shot personalized sketch segmentation is however non-trivial. 
The key challenge lies with deriving means \old{of effectively transferring}\new{to efficiently transfer} the semantic labels in the exemplar to all target sketches so that parts semantics are preserved. 
Diversity in sketch depictions among humans (e.g., the ducks in Fig.~\ref{fig:teaser}) makes this task even more challenging.


In our work, we exploit \emph{deformation}, and train the segmentation module by morphing the exemplar sketch to available sketches of a given category. 
To increase robustness, we propose a hierarchical deformation model specific to sketch data. During training, we first globally align all sketches with the exemplar\new{,} and then \old{obtain}\new{predict} a fine-level warping of the exemplar towards \old{the}\new{each of} globally aligned sketches.
Such an approach simplifies the task of the segmentation network: The segmentation network does not need to deal with large geometric differences.
\old{At inference time}\new{During inference}, we first perform a global alignment with the exemplar, then \new{we} predict the segmentation and\new{,} finally \new{we} apply an inverse global transformation operator.


Our first key contribution is in exploiting the connectivity information encoded in sketch strokes, in both parts of our segmentation model: deformation and segmentation. To embed this information we obtain a multi-level sketch encoding using a graph convolution network (GCN). The graph consists of dynamic and static edges. The role of dynamic edges is to encode global information embedded into the holistic sketch. The static edges connect the consequent points along strokes, encoding stroke-level information. \old{Such representation allows to retain both sketch- and stroke-level embeddings in a synergistic fashion.}



The sketch deformation module, \old{being}\new{which is} our central contribution, builds around this sketch representation. On the holistic sketch level, we first predict a global rigid-body transformation with respect to an exemplar sketch, relying on an analytic solver. 
We observe that the conventional Chamfer distance \cite{wang2020few,yuan2020ross} between an input sketch and an exemplar is not sufficient to predict the global transformation which preserves semantic part correspondences, due to the sparse nature of sketches. 
We instead jointly train for unsupervised keypoints prediction \cite{chen2020unsupervised} which are used to derive global transformation. 
Such rigid-body deformation however only \textit{roughly} aligns the gallery sketch to the exemplar. 
To achieve finer alignment, \old{we impose stroke-level deformations rather than individually on stroke points}\new{we apply deformations at the stroke level, and not individually on the stroke points}. 
To avoid unrealistic stroke distortions\new{,} we limit the transformations to \old{stroke-level} rotation, translation\new{,} and scaling \new{at the stroke level}. 
To achieve a globally consistent deformation \old{on}\new{at} this level, we leverage both Chamfer distance and mean square error \new{computed} on keypoints \new{positions}. 
The distances are computed between the \new{keypoints of the} fine-level deformed exemplar and a holistic sketch-level deformed gallery sketch.



Given the deformed exemplar\new{,} we train a segmentation module in a standard fashion via a cross-entropy loss, which given the full sketch encoding predicts a label for each sketch point. We \old{further}\new{also} observe that sketch strokes are frequently \old{fully}\new{completely} contained within one semantic part. 
\old{We thus}\new{Therefore, we} further condition the segmentation label predictor on the stroke encoding, eliminating the need for a labels refinement step such as graph-cuts \cite{li2018fast} or conditional random fields \cite{schneider2016example, zhu20202d}.


In summary, (i) we propose for the first time the problem of one-shot sketch segmentation; (ii) we show that by transferring the semantic labeling from an input sketch to target ones, a much-desired personalized segmentation capability can be achieved; (iii) we propose a hierarchical sketch deformation framework that faithfully deforms the input sketch to each reference, as means to assist the transfer; (iv)  we conduct multiple ablation studies demonstrating the robustness of our proposed method in terms of variations in part semantics and sketching style; (v) we show an advantage of our method over alternative solutions for a few-shot sketch segmentation.





==> related_work.tex <==
\section{Related work}

\label{sec:related_work}
% -------------------------------------
% Sketch segmentation
% -------------------------------------
\paragraph{Sketch segmentation}
Prior works on sketch segmentation can be divided into two categories based on the segmentation goals: strokes perceptual grouping \cite{qi2013sketching, qi2015making, li2018universal, liu2018strokeaggregator} and semantic segmentation 
\cite{sun2012free, huang2014data, schneider2016example, zhu2018part, li2018fast, wu2018sketchsegnet, wang2018sketchpointnet,  li2019toward, qi2019sketchsegnet+, wang2019spfusionnet, hahnlein2019bitmap, yang2020sketchgcn, zhu2020sketchppnet}.
Our work belongs to the second category. \old{Yet, we}\new{However}, for the first time, \new{we} consider the problem of \old{a }\emph{one-shot} semantic sketch segmentation.



% Datasets:
\old{A}\new{The a}ppearance of large-scale annotated sketch datasets \cite{huang2014data, li2018universal, eitz2012humans, li2018fast} fostered research on supervised semantic sketch segmentation \old{with}\new{using} deep learning.
These methods can be classified into several groups \old{by the used sketch representation}\new{according to the sketch representation used}: 
image-based  \cite{li2018fast, zhu20202d, ge2020creative},
point-based  \cite{ hahnlein2019bitmap, wang2020multi},
ordered point sequences-based \cite{wu2018sketchsegnet, qi2019sketchsegnet+}, 
joint pixel-/point-based \cite{wang2019spfusionnet} methods,
and graph-based \cite{yang2020sketchgcn}.
%
\emph{Image-based} methods represent a sketch as a raster image\old{,} and build on \old{a}\new{the} success of convolutional neural networks (CNNs) in learning descriptive features. 
Zhu et al.~\cite{zhu20202d} combine\anran{d} a CNN-based segmentation with \old{a }CRF-based \old{refining}\new{refinement}.
%
\emph{Point-based} methods \cite{ hahnlein2019bitmap, wang2020multi} represent\anran{ed} a sketch as an ordered point cloud. 
Such works \old{build}\anran{built} on the point-cloud architectures, first designed for \new{the} 3D shape analysis and representation \cite{qi2017pointnet, qi2017pointnet++, li2018pointcnn, wang2019dynamic}. 
Point-based representation \old{allows to reduce models complexity,}\new{reduces the complexity of models} compared to image\old{d}-based representations\old{,} due to the sparsity of lines in sketches. 
For the task of sketch recognition, Wang et al.~\cite{wang2018sketchpointnet} proposed a sketch-dedicated point cloud architecture. 
Both Wang et al.~\cite{wang2018sketchpointnet} and Hahnlein et al.~\cite{ hahnlein2019bitmap} \old{take}\anran{took} as points features not only \new{the} points spatial coordinates\old{,} but also \new{the} strokes order.
%
A number of works \cite{wu2018sketchsegnet, qi2019sketchsegnet+,yang2020s} exploit\anran{ed} \emph{recurrent neural networks (RNNs)} to translate sequence of strokes into their semantic parts. 
Such architectures were first designed for \old{the }the task of sketch recognition \cite{ha2017neural, li2018sketch, jia2020coupling}. 
\old{We though}\new{However, we} did not observe a correlation between a semantic stroke label and a stroke number in \old{a}\new{the} general case.
%
Wang et al.~\cite{wang2019spfusionnet} \emph{\old{fuses}} \emph{\anran{fused}} a prediction of \old{the}\new{a} dedicated image-based architecture with the one obtained from a point-based architecture \cite{qi2017pointnet}. 
Recently, Zhu et al.~\cite{zhu2020sketchppnet} applied a similar idea to \old{a}\new{the} sketch recognition task.
%
\old{Despite \emph{graph-based} sketch representation was commonly used in earlier works on sketch analysis, just recently graph convolution networks (GCNs) were adopted for sketch processing.}
\new{While earlier sketch analysis work commonly used \emph{graph-based} representation of sketches, it is only recently that Graph Convolution Networks (GCNs) have been adopted for sketch processing.}
Yang et al.~\cite{yang2020sketchgcn} proposed a two branches GCN for a supervised sketch segmentation task, implementing graph convolutions as was proposed in \cite{wang2019dynamic} and \cite{li2019deepgcns}.
Su et al.~\cite{su2020sketchhealer} exploited GCN with a sparse number of nodes for the partial sketch completion task.
Yang et al.~\cite{yang2020s} leverage\anran{d} \new{a} RNN \old{with}\new{in} conjunction with \new{a} GCN for \old{a }sketch recognition\old{ task}.
%
In our work, we \old{leverage}\new{employ} a GCN for \old{the task of a }few-shot sketch segmentation, leveraging a multilevel sketch encoding.

% -------------------------------------
% 3D shape segmentation
% -------------------------------------

\paragraph{3D shape segmentation}
Concurrently, two approaches for \old{a }few-shot 3D shape segmentation \old{were}\new{have} recently \new{been} proposed \cite{yuan2020ross, wang2020few}, relying on the idea of being able to morph a template shape to an arbitrary target shape. 
Yuan et al.~\cite{yuan2020ross} directly transfer\old{s}\anran{ed} a label from the morphed template to the target shape by proximity. 
Wang et al.~\cite{wang2020few} instead learn\old{s}\anran{ed} a continuous probability distribution function that learns to assign to each point in space \old{a}\new{the} probability of having a certain semantic label\old{,} conditioned on a global shape feature vector. 
Yuan et al.~\cite{yuan2020ross} exploit\anran{ed} mesh connectivity, while Wang et al.~\cite{wang2020few} \old{rely}\anran{relied} on a point-based shape representation.

Chen et al.~\cite{chen2019bae} proposed an autoencoder for unsupervised consistent segmentation of shapes from the same class\old{,} and demonstrated how such \new{an} architecture can be \old{tuned}\new{repurposed} for one-shot learning. 
The autoencoder consist\new{s} of several branches\old{, which} \new{that} are trained to encode complementary shape parts.
Instead of decomposing the shape into parts, Chen et al.~\cite{chen2020unsupervised} stud\old{y}\anran{ied} the problem of unsupervised prediction of semantically \old{consist}\new{consistent} keypoints across all shapes of the same class. 
Dense predicted keypoints correspondences are used to transfer semantic labels from one shape to another.

Our work extends these ideas to \old{a} few-shot sketch segmentation, taking into account point\old{s} connectivity and sketch sparsity, designed to be robust to arbitrary global sketch rotation and reflection. 
